Unsupervised Word Translation Pairing using Refinement based Point Set Registration

Cross-lingual alignment of word embeddings play an important role in knowledge transfer across languages, for improving machine translation and other multi-lingual applications. Current unsupervised approaches rely on similarities in geometric structure of word embedding spaces across languages, to learn structure-preserving linear transformations using adversarial networks and refinement strategies. However, such techniques, in practice, tend to suffer from instability and convergence issues, requiring tedious fine-tuning for precise parameter setting. This paper proposes BioSpere, a novel framework for unsupervised mapping of bi-lingual word embeddings onto a shared vector space, by combining adversarial initialization and refinement procedure with point set registration algorithm used in image processing. We show that our framework alleviates the shortcomings of existing methodologies, and is relatively invariant to variable adversarial learning performance, depicting robustness in terms of parameter choices and training losses. Experimental evaluation on parallel dictionary induction task demonstrates state-of-the-art results for our framework on diverse language pairs.

==> rel.tex <==
\section{Related Work}
\label{sec:rel}

{\bf Generative Adversarial Networks} (GANs) couples the training of machine learning architecture between a {\em generative} and a {\em discriminative} network that work in tandem for ``indirect'' training in an 
unsupervised manner~\cite{gan}. GANs have been shown to achieve impressive results in the domain image processing~\cite{cgan}, representation learning~\cite{rep} and reinforcement learning~\cite{ho16}. The idea of
{\em adversarial loss} is particularly useful for image processing task like image generation, image in-painting, and image translation. The task of image-to-image translation involves learning the transformation from 
an input image to an output image, based on annotated image pairs~\cite{pair}. However, to alleviate the problem of large annotated dataset required for training, unpaired image-to-image translation approach, 
Co-GAN~\cite{cogan} was proposed based on weight sharing scheme to learn a common mapping. Removal of dependencies on task-specific similarity functions and low-dimensionality in this aspect, was proposed by~\citet{cgan} 
by use of transitivity to regularize structured data, as was shown in visual tracking by enforcing forward-backward consistency~\cite{track}. Interestingly, verifying and improving translations via ``back translation and 
reconciliation'' is a technique used by human translators as reported in~\cite{lang}. In this context, we thus adopt the unsupervised CycleGAN~\cite{cgan} adversarial training architecture based on the cycle-consistency 
loss (for image pairing) to find word correspondence across different language embedding spaces.

{\bf Point Set Registration.}

